QiMeng-CodeV-SVA: Training Specialized LLMs for Hardware Assertion Generation via RTL-Grounded Bidirectional Data Synthesis

SystemVerilog Assertions (SVAs) are crucial for hardware verification. Recent studies leverage general-purpose LLMs to translate natural language properties to SVAs (NL2SVA), but they perform poorly due to limited data. We propose a data synthesis framework to tackle two challenges: the scarcity of high-quality real-world SVA corpora and the lack of reliable methods to determine NL-SVA semantic equivalence. For the former, large-scale open-source RTLs are used to guide LLMs to generate real-world SVAs; for the latter, bidirectional translation serves as a data selection method. With the synthesized data, we train CodeV-SVA, a series of SVA generation models. Notably, CodeV-SVA-14B achieves 75.8% on NL2SVA-Human and 84.0% on NL2SVA-Machine in Func.@1, matching or exceeding advanced LLMs like GPT-5 and DeepSeek-R1.

==> sections/3_background.bk.tex <==
\section{Problem Statement}
\label{sec:background}

We formally describe the NL2SVA task discussed in this paper as follows:

\begin{definition}[LLM-based NL-to-SVA Translation]
\label{def:NL2SVA}
Given an under-test RTL design code $\mathbf{c}$ and a natural-language verification property $\mathbf{x}$ as inputs to an LLM $\mathcal{M}$, the model outputs a SystemVerilog Assertion (SVA) $\mathbf{y}$, optionally accompanied by a reasoning process. We say that $\mathbf{y}$ is a correct NL-to-SVA translation of $\mathbf{x}$ with respect to $\mathbf{c}$, if and only if:

(1) \textbf{Syntax Correctness}: $\mathbf{y}$ conforms to the syntax of SVA.

(2) \textbf{Functional Correctness}: $\mathbf{y}$ is semantically equivalent to $\mathbf{x}$ with respect to $\mathbf{c}$.

\end{definition}



==> sections/5_implementation_details.tex <==
 

==> tables/5_experiments/assertionforge.bk.tex <==
\begin{table*}[h]
\centering
\caption{Evaluation results. 
         (\#SVA: total assertions generated; \#SynC: syntactically correct; \#Proven: proven or passing;
          COI Statement/Branch/Functional/Toggle: coverage metrics for each coverage model under COI.)}
\label{tab:results}
\begin{tabular}{llccccccc}
\toprule
\multirow{2}{*}{Spec2NL} & \multirow{2}{*}{NL2SVA} & \multirow{2}{*}{\#SVA} & \multirow{2}{*}{\#SynC} & \multirow{2}{*}{\#Proven} 
  & \multicolumn{4}{c}{COI Coverage (\%)} \\
\cline{6-9}
& & & & & Statement & Branch & Functional & Toggle \\
\hline
\multicolumn{8}{c}{\textsc{APB}} \\
\hline
GPT-4o  & GPT-4o         & 436 & 377 & 106 & 100.00 & 100.00 & 100.00 & 100.00 \\
GPT-4o  & \modelname-8B  & 442 & 384 & 180 & 100.00 & 100.00 & 100.00 & 100.00 \\
GPT-4o  & \modelname-14B & 437 & 395 & 151 & 100.00 & 100.00 & 100.00 & 100.00 \\
\hline
\RR     & \RR            & 515 & 281 & 122 & 100.00 & 100.00 & 100.00 & 100.00 \\
\RR     & \modelname-8B  & 529 & 466 & 211 & 100.00 & 100.00 & 100.00 & 100.00 \\
\RR     & \modelname-14B & 512 & 445 & 175 & 100.00 & 100.00 & 100.00 & 100.00 \\
\hline

\multicolumn{8}{c}{\textsc{ETHMAC}} \\
\hline
GPT-4o  & GPT-4o         & 720 & 565 & 49 & 100.00 & 100.00 & 99.87 & 99.80 \\
GPT-4o  & \modelname-8B  & 721 & 579 & 76 & 100.00 & 100.00 & 99.87 & 99.80 \\
GPT-4o  & \modelname-14B & 715 & 580 & 71 & 100.00 & 100.00 & 99.87 & 99.80 \\
\hline
\RR     & \RR            & 665 & 371 & 75 & 100.00 & 100.00 & 99.87 & 99.80 \\
\RR     & \modelname-8B  & 660 & 532 & 84 & 100.00 & 100.00 & 99.87 & 99.80 \\
\RR     & \modelname-14B & 632 & 510 & 85 & 100.00 & 100.00 & 99.87 & 99.80 \\
\hline

\multicolumn{8}{c}{\textsc{OPENMSP430}} \\
\hline
GPT-4o  & GPT-4o         & 1013 & 777 & 196 & 100.00 & 100.00 & 90.66 & 88.96 \\
GPT-4o  & \modelname-8B  & 1044 & 859 & 484 & 100.00 & 100.00 & 91.10 & 89.48 \\
GPT-4o  & \modelname-14B & 1029 & 829 & 454 & 100.00 & 100.00 & 91.10 & 89.48 \\
\hline
\RR     & \RR            & 1222 & 496 & 144 & 100.00 & 99.65  & 90.46 & 88.76 \\
\RR     & \modelname-8B  & 1215 & 917 & 502 & 100.00 & 100.00 & 91.10 & 89.48 \\
\RR     & \modelname-14B & 1192 & 916 & 482 & 100.00 & 100.00 & 91.10 & 89.48 \\
\hline

\multicolumn{8}{c}{\textsc{SOCKIT}} \\
\hline
GPT-4o  &  GPT-4o        & 251 & 173 & 31 & 100.00 & 100.00 & 99.73 & 99.60 \\
GPT-4o  & \modelname-8B  & 251 & 202 & 49 & 100.00 & 100.00 & 99.73 & 99.60 \\
GPT-4o  & \modelname-14B & 258 & 208 & 50 & 100.00 & 100.00 & 99.73 & 99.60 \\
\hline
\RR     & \RR            & 232 & 122 & 40 & 100.00 & 100.00 & 99.73 & 99.60 \\
\RR     & \modelname-8B  & 247 & 178 & 58 & 100.00 & 100.00 & 99.73 & 99.60 \\
\RR     & \modelname-14B & 234 & 184 & 53 & 100.00 & 100.00 & 99.73 & 99.60 \\
\hline

\multicolumn{8}{c}{\textsc{UART}} \\
\hline
GPT-4o  & GPT-4o         & 265 & 186 & 54 & 100.00 & 100.00 & 100.00 & 100.00 \\
GPT-4o  & \modelname-8B  & 270 & 196 & 73 & 100.00 & 100.00 & 100.00 & 100.00 \\
GPT-4o  & \modelname-14B & 281 & 182 & 68 & 100.00 & 100.00 & 100.00 & 100.00 \\
\hline
\RR     & \RR            & 258 & 91  & 40 & 100.00 & 100.00 & 100.00 & 100.00 \\
\RR     & \modelname-8B  & 266 & 185 & 70 & 100.00 & 100.00 & 100.00 & 100.00 \\
\RR     & \modelname-14B & 275 & 176 & 70 & 100.00 & 100.00 & 100.00 & 100.00 \\
\bottomrule


\end{tabular}
\end{table*}


==> tables/5_experiments/assertionforge_with_coi.tex <==
\begin{table*}[h]
\centering
\caption{Evaluation results. 
         (\#SVA: total assertions generated; \#SynC: syntactically correct; \#Proven: proven or passing;
          COI Statement/Branch/Functional/Toggle: coverage metrics for each coverage model under COI.)}
\label{tab:results}
\begin{tabular}{llccccccc}
\toprule
\multirow{2}{*}{Spec2NL} & \multirow{2}{*}{NL2SVA} & \multirow{2}{*}{\#SVA} & \multirow{2}{*}{\#SynC} & \multirow{2}{*}{\#Proven} 
  & \multicolumn{4}{c}{COI Coverage (\%)} \\
\cline{6-9}
& & & & & Statement & Branch & Functional & Toggle \\
\hline
\multicolumn{8}{c}{\textsc{APB}} \\
\hline
GPT-4o  & GPT-4o                    & 436 & 377 & 106 & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} \\
\rowcolor[rgb]{0.925,0.925,0.925} GPT-4o  & \modelname-8B (ours)      & \textbf{442} & \textbf{384} & \textbf{180} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} \\
\hline
\RR     & \RR                       & 515 & 281 & 122 & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} \\
\rowcolor[rgb]{0.925,0.925,0.925} \RR     & \modelname-8B (ours)      & \textbf{529} & \textbf{466} & \textbf{211} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} \\
\hline

\multicolumn{8}{c}{\textsc{ETHMAC}} \\
\hline
GPT-4o  & GPT-4o         & 720 & 565 & 49 & \textbf{100.00} & \textbf{100.00} & \textbf{99.87} & \textbf{99.80} \\
\rowcolor[rgb]{0.925,0.925,0.925} GPT-4o  & \modelname-8B (ours)  & \textbf{721} & \textbf{579} & \textbf{76} & \textbf{100.00} & \textbf{100.00} & \textbf{99.87} & \textbf{99.80} \\
\hline
\RR     & \RR            & \textbf{665} & 371 & 75 & \textbf{100.00} & \textbf{100.00} & \textbf{99.87} & \textbf{99.80} \\
\rowcolor[rgb]{0.925,0.925,0.925} \RR     & \modelname-8B (ours)  & 660 & \textbf{532} & \textbf{84} & \textbf{100.00} & \textbf{100.00} & \textbf{99.87} & \textbf{99.80} \\
\hline

\multicolumn{8}{c}{\textsc{OPENMSP430}} \\
\hline
GPT-4o  & GPT-4o         & 1013 & 777 & 196 & \textbf{100.00} & \textbf{100.00} & 90.66 & 88.96 \\
\rowcolor[rgb]{0.925,0.925,0.925} GPT-4o  & \modelname-8B (ours) & \textbf{1044} & \textbf{859} & \textbf{484} & \textbf{100.00} & \textbf{100.00} & \textbf{91.10} & \textbf{89.48} \\
\hline
\RR     & \RR            & \textbf{1222} & 496 & 144 & \textbf{100.00} & 99.65  & 90.46 & 88.76 \\
\rowcolor[rgb]{0.925,0.925,0.925} \RR     & \modelname-8B (ours) & 1215 & \textbf{917} & \textbf{502} & \textbf{100.00} & \textbf{100.00} & \textbf{91.10} & \textbf{89.48} \\
\hline

\multicolumn{8}{c}{\textsc{SOCKIT}} \\
\hline
GPT-4o  &  GPT-4o        & \textbf{251} & 173 & 31 & \textbf{100.00} & \textbf{100.00} & \textbf{99.73} & \textbf{99.60} \\
\rowcolor[rgb]{0.925,0.925,0.925} GPT-4o  & \modelname-8B (ours)  & \textbf{251} & \textbf{202} & \textbf{49} & \textbf{100.00} & \textbf{100.00} & \textbf{99.73} & \textbf{99.60} \\
\hline
\RR     & \RR            & 232 & 122 & 40 & \textbf{100.00} & \textbf{100.00} & \textbf{99.73} & \textbf{99.60} \\
\rowcolor[rgb]{0.925,0.925,0.925} \RR     & \modelname-8B (ours)  & \textbf{247} & \textbf{178} & \textbf{58} & \textbf{100.00} & \textbf{100.00} & \textbf{99.73} & \textbf{99.60} \\
\hline

\multicolumn{8}{c}{\textsc{UART}} \\
\hline
GPT-4o  & GPT-4o         & 265 & 186 & 54 & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} \\
\rowcolor[rgb]{0.925,0.925,0.925} GPT-4o  & \modelname-8B (ours)  & \textbf{270} & \textbf{196} & \textbf{73} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} \\
\hline
\RR     & \RR            & 258 & 91  & 40 & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} \\
\rowcolor[rgb]{0.925,0.925,0.925} \RR     & \modelname-8B (ours)  & \textbf{266} & \textbf{185} & \textbf{70} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} \\
\bottomrule


\end{tabular}
\label{tab:assertionforge}
\end{table*}


==> tables/5_experiments/main_results.bk.tex <==
\begin{table*}[t]
\centering
%\setlength{\tabcolsep}{1mm}
%\fontsize{9}{11}\selectfont
\caption{TODO}
\begin{tabular}{l|ccc|ccc}
\toprule
\multirow{2}{*}{Method}     & \multicolumn{3}{c}{\HUMAN} & \multicolumn{3}{c}{\MACHINE} \\
                    & Func.@1    & Func.@16   & Func.@32  & Func.@1  & Func.@16  & Func.@32   \\
\midrule
\RR                 & 74.6       & 90.3       & 90.4      & 81.0     & 93.3      & 94.3 \\
GPT-5               & 71.8       & 90.2       & 92.7      & 81.8     & 93.2      & 94.3 \\
\VV                 & 63.1       & 81.4       & 84.9      & 83.8     & 92.9      & 93.6 \\
GPT-4o              & 64.1       & 75.2       & 78.1      & 68.5     & 81.3      & 83.7 \\
\midrule
Qwen3-8B            & 32.3       & 71.6       & 74.0      & 46.1     & 88.0      & 90.5 \\
Qwen3-14B           & 61.6       & 86.1       & 87.7      & 75.3     & 92.7      & 94.3 \\
\midrule
\modelname-8B       & 72.0       & 88.8       & 90.4      & 83.5     & 96.3      & 97.2 \\
\modelname-14B      & 75.8       & 89.4       & 90.4      & 84.0     & 94.9      & 95.8 \\
\bottomrule
\end{tabular}
\label{tab:main_results}
\end{table*}
